Structured adaptive and random spinners for fast machine learning computations

We consider an efficient computational framework for speeding up several machine learning algorithms with almost no loss of accuracy. The proposed framework relies on projections via structured matrices that we call Structured Spinners, which are formed as products of three structured matrix-blocks that incorporate rotations. The approach is highly generic, i.e. i) structured matrices under consideration can either be fully-randomized or learned, ii) our structured family contains as special cases all previously considered structured schemes, iii) the setting extends to the non-linear case where the projections are followed by non-linear functions, and iv) the method finds numerous applications including kernel approximations via random feature maps, dimensionality reduction algorithms, new fast cross-polytope LSH techniques, deep learning, convex optimization algorithms via Newton sketches, quantization with random projection trees, and more. The proposed framework comes with theoretical guarantees characterizing the capacity of the structured model in reference to its unstructured counterpart and is based on a general theoretical principle that we describe in the paper. As a consequence of our theoretical analysis, we provide the first theoretical guarantees for one of the most efficient existing LSH algorithms based on the HD3HD2HD1 structured matrix [Andoni et al., 2015]. The exhaustive experimental evaluation confirms the accuracy and efficiency of structured spinners for a variety of different applications.

==> applications.tex <==
\section{Computing general kernels with Structured Spinners}
\label{sec:applications}
% We start with the following result characterizing continuous positive definite shift-invariant kernels.
% \begin{theorem}[Bochner]
% A continuous kernel $k(\textbf{x},\textbf{y}) = g(\textbf{x} - \textbf{y})$ on $\mathbb{R}^{d}$ is positive definite if and only if $g(\delta)$ is a Fourier transform of a non-negative measure, i.e.:
% \begin{equation}
% k(\textbf{x},\textbf{y}) = \int_{\mathbb{R}^{d}} p(\omega)e^{i\omega^\top\cdot (\textbf{x}-\textbf{y})} d \omega = \mathbb{E}_{\omega}[\xi_{\omega}(\textbf{x}) \xi_{\omega}(\textbf{y})^{*}],
% \end{equation}
% \end{theorem}
% for the non-negative measure $p$ on $\mathbb{R}^{d}$ and $\xi_{\omega}(\textbf{x}) = e^{i \omega^\top \cdot \textbf{x}}$.
% That result, interpreted in the Monte-Carlo approximation setup leads to the unbiased estimations of various kernels $k(\textbf{x},\textbf{y})$ by a sum of the normalized dot products $\frac{1}{k}f(\textbf{P} \textbf{x})^\top\cdot f(\textbf{P} \textbf{y})$, where $\textbf{P} \in \mathbb{R}^{k \times d}$ is a random matrix related to the non-negative measure $p$, $f$ is a fixed nonlinear function $\mathbb{R} \rightarrow \mathbb{R}$ and $f(\textbf{v})$ for $\textbf{v}=(v_{1},...,v_{k})^\top \in \mathbb{R}^{k}$ is defined as 
% $f(\textbf{v}) = (f(v_{1}),...,f(v_{k}))^\top$ \cite{rahimi}.
% In the case of the Gaussian kernel $\textbf{P}$ is Gaussian and matrices from the $3StructBlock$-family can replace $\textbf{P}$ to speed up computations and reduce storage complexity. As we will show below, this same technique can be used to efficiently evaluate a wide range of kernels.

% For certain kernels matrices $\textbf{P}$ are Gaussian (see: Table \ref{tab:literature}). This is the case for instance for Gaussian kernels (where the nonlinear mappings are: $\sin$ and $\cos$ functions) for the angular kernel (where $f$ is a Heaviside step function) and for arc-cosine kernels (where $f$ is a ReLU function). In these settings matrices from the $3StructBlock$-family can replace $\textbf{P}$ to speed up computations of these kernels and reduce storage complexity.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsubsection{PNG Kernels}
Previous works regarding approximating kernels with structured matrices covered only some special kernels, namely: Gaussian, arc-cosine and angular kernels.
We explain here how structured approach (in particular our \textit{TripleSpin}-family) can be used to approximate well most kernels.
Theoretical guarantees that cover also this special case are given in the subsequent section.

For kernels that can be represented as an expectation of Gaussian random variables it is natural to approximate them using structured matrices. We start our analysis with the so-called \textit{Pointwise Nonlinear Gaussian kernels (PNG)} which are of the form:
\vspace{-0.28in}
% We will use \textit{Pointwise Nonlinear Gaussian kernels (PNGs)} as building blocks in our structured approximations of kernels.
% A PNG is of the form:
\begin{equation}
\label{eq:main_function_simple}
\kappa_{f,\mu,\Sigma}(\textbf{x},\textbf{y}) = \mathbb{E}\left[f(\textbf{g}^\top \cdot \textbf{x})\cdot f(\textbf{g}^\top \cdot \textbf{y})\right]
\vspace{-0.3in}
\end{equation}
where: $\textbf{x},\textbf{y} \in \mathbb{R}^{n}$, the expectation is over a multivariate Gaussian $\textbf{g}\sim\mathcal{N}(\mu,\Sigma)$ and $f$ is a fixed nonlinear function $\mathbb{R} \rightarrow \mathbb{R}$ (the positive-semidefiniteness of the kernel follows from it being an expectation of dot products). 
The expectation, interpreted in the Monte-Carlo approximation setup, leads to an unbiased estimation by a sum of the normalized dot products $\frac{1}{k}f(\textbf{G} \textbf{x})^\top\cdot f(\textbf{G} \textbf{y})$, where $\textbf{G} \in \mathbb{R}^{k \times n}$ is a random Gaussian matrix and $f$ is applied pointwise, i.e. $f((v_{1},...,v_{k})):=(f(v_{1}),...,f(v_{k}))$. 

In this setting matrices from the $TripleSpin$-family can replace $\textbf{G}$ with diagonal covariance matrices $\Sigma$ to speed up computations and reduce storage complexity. 
This idea of using random structured matrices to evaluate such kernels is common in the literature, e.g. \cite{choromanska2015binary,le2013fastfood}, but no theoretical guarantees were given so far for general PNG kernels (even under the restriction of diagonal $\Sigma$).

PNGs define a large family of kernels characterized by $f,\mu,\Sigma$. 
%Prominent examples, including the Euclidean and angular distance, are given in Table~\ref{tab:literature}.
Prominent examples include the Euclidean and angular distance \cite{choromanska2015binary}, the arc-cosine kernel \cite{NIPS2009_3628} and the sigmoidal neural network~\cite{Williams:1998:CIN:295919.295941}. 
Since sums of kernels are again kernels, we can construct an even larger family of kernels by summing PNGs. A simple example is the Gaussian kernel which can be represented as a sum of two PNGs with $f$ replaced by the trigonometric functions: $\sin$ and $\cos$.
%\begin{align*}
%\kappa_{G}(\textbf{x},\textbf{y}) &= \exp\left(-\|\textbf{x}-%\textbf{y}\|^{2}_2/2\right) =  \mathbb{E}\left[\cos( %\textbf{g}^\top\cdot \textbf{x})\cos( \textbf{g}^\top \cdot %\textbf{y})\right]
% +\mathbb{E}\left[\sin( \textbf{g}^\top\cdot \textbf{x})\sin( %\textbf{g}^\top\cdot \textbf{y})\right]
%\end{align*}
%with $\textbf{g}\sim\mathcal{N}(0,I)$. 

Since the Laplacian, exponential and rational quadratic kernel can all be represented as a mixture of
Gaussian kernels with different variances,
%\todo{Francois}{Please define or rephrase scale mixture here. I presume it means a mixture of Gaussians with different variances.}
they can be easily approximated by a finite sum of PNGs. Remarkably, virtually all kernels can be represented as a (potentially infinite) sum of PNGs with diagonal $\Sigma$.
Recall that kernel $\kappa$ is stationary if $\kappa(x,y)=\kappa(x-y)$ for all $x,y \in \mathbb{R}^{n}$ and non-stationary otherwise.
Harnessing Bochner's and Wiener’s Tauberian theorem~\cite{samo2015generalized}, we show that all stationary kernels may be approximated arbitrarily well by sums of PNGs. 
% \begin{table}[t!]
% \renewcommand{\arraystretch}{1.35}
% \centering
%  \begin{tabular}{|c |c | c | } 
% 
%  \hline
%  \bf{Kernel name} & $f(x)$ & $\kappa_{f,\mu,\Sigma}$  \\
%  \hline \hline
% 
% Euclidean distance & $x$ & $ \textbf{x}^\top\cdot\textbf{y}$ \\ \hline
% 
% Angular distance \cite{choromanska2015binary} & $\Theta(x)$ & $\frac{1}{2\pi}(\pi-\theta_{\textbf{x},\textbf{y}})$ \\ \hline
% 
% Arc-cosine \cite{NIPS2009_3628} & $\Theta(x)x^b$  & $\frac{1}{2\pi}||\textbf{x}||^b||\textbf{y}||^bJ_b(\theta_{\textbf{x},\textbf{y}})$ \\ \hline
%
% Sigmoidal neural network \cite{Williams:1998:CIN:295919.295941} & $\mbox{erf}(x)$  & $\frac{2}{\pi}\arcsin\left( \frac{2 \textbf{x}^\top\Sigma \textbf{y}}{\sqrt{\left(1+2\textbf{x}^\top\Sigma \textbf{x}\right)\left(1+2\textbf{y}^\top\Sigma \textbf{y}\right)}} \right)$   \\ \hline
%
% % Neural network: Gaussian pdf \cite{Williams:1998:CIN:295919.295941} & $\phi(x)$  & $3^{-d/2}\phi(\textbf{x}/\sqrt{3})\phi((\textbf{x}-\textbf{y})/\sqrt{3})\phi(\textbf{y}/\sqrt{3})$   \\ \hline
% \end{tabular}
% 
% \vspace{0.25cm}
% \caption{PNGs in the literature. Here $\mu = 0$ always, $\Sigma = I$ except for the sigmoidal neural network, $\theta_{\textbf{x},\textbf{y}}$ is the angle between $\textbf{x}$ and $\textbf{y}$, $\Theta$ is the heaviside step function and $\mbox{erf}$ is the error function.  The definition of $J_{b}(\theta_{\textbf{x},\textbf{y}})$) is given in \cite{NIPS2009_3628}.
% } \label{tab:literature}
% \vspace{-0.5cm}
% \end{table}
%
%\todo{Francois}{Could you replace dimension $d$ with $n$ here and in the appendix to match Krzysztof's proofs? I suggest we omit all $2\pi$ from statement of Thm 1 and 2, as those can be absorbed into $\sigma$ and $w$? Could we drop $+$ from $\mathbb{R}^{d+}$ as $d+$ is undefined, would need space we are tight on and it's correct without it? Similarly can we write $\mathbb{N}\cup\{\infty\}$ in place of $\mathbb{N}^*$? Lastly, what's known about the rate of convergence in these statements, if any?}
% I have made the suggested changes. There are some rates like in "RATES OF CONVERGENCE FOR THE GAUSSIAN MIXTURE SIEVE", but they do not consider the data and hence are not particularly useful to us. I am not aware of any convergence result that relies on the data, but will look for one.
\begin{comment}
\begin{theorem}[stationary kernels] 
\label{thm:stationary}
The family of functions
\begin{align*}
\kappa_K(\textbf{x},\textbf{y})&:=\sum_{k=1}^K\alpha_k (\mathbb{E}[\cos(\textbf{g}_k^\top\cdot \textbf{x})\cos(\textbf{g}_k^\top\cdot \textbf{y})] + \mathbb{E}[\sin(\textbf{g}_k^\top\cdot \textbf{x})\sin(\textbf{g}_k^\top\cdot \textbf{y})])
\end{align*}
with $\textbf{g}_k\sim\mathcal{N}(\mu_k,\mbox{diag}((\sigma_{k}^1)^2,...,(\sigma_k^d)^2))$, $\mu_k,\sigma_k\in\mathbb{R}^{n}$, $\alpha_k\in\mathbb{R}$, $K\in\mathbb{N}\cup\{\infty\}$ is dense in the family of stationary real-valued kernels with respect to pointwise convergence.
\end{theorem}
\end{comment}
%\vspace{-0.05in}
\begin{theorem}[stationary kernels] 
\label{thm:stationary}
The family of functions 
\begin{align*}
\kappa_K(\textbf{x},\textbf{y}):=\sum_{k=1}^K\alpha_k ( A + B), \\
A = \mathbb{E}[\cos(\textbf{g}_k^\top\cdot \textbf{x})\cos(\textbf{g}_k^\top\cdot \textbf{y})], \\
B = \mathbb{E}[\sin(\textbf{g}_k^\top\cdot \textbf{x})\sin(\textbf{g}_k^\top\cdot \textbf{y})]
\end{align*}

with $\textbf{g}_k\sim\mathcal{N}(\mu_k,\mbox{diag}((\sigma_{k}^1)^2,...,(\sigma_k^d)^2))$, $\mu_k,\sigma_k\in\mathbb{R}^{n}$, $\alpha_k\in\mathbb{R}$, $K\in\mathbb{N}\cup\{\infty\}$ is dense in the family of stationary real-valued kernels with respect to pointwise convergence.
\end{theorem}

This family corresponds to the \textit{spectral mixture kernels} of \cite{wilson2013gaussian}. We can extend these results to arbitrary, non-stationary, kernels; the precise statement and its proof can be found in the Appendix.

Theorem \ref{thm:stationary} and its non-stationary analogue show that the family of sums of PNGs contains virtually all kernel functions. If a kernel can be well approximated by the sum of only a small number of PNGs then we can use the $TripleSpin$-family to efficiently evaluate it. It has been found in the Gaussian Process literature that often a small sum of kernels tuned using training data is sufficient to explain phenomena remarkably well \cite{wilson2013gaussian}. The same should also be true for the sum of PNGs. This suggests a methodology for learning the parameters of a sum of PNGs from training data and then applying it out of sample. %The parameters of the PNG sum could be fit by nonlinear conjugate gradients as it is for Gaussian Processes \cite{wilson2013gaussian}. 
We leave this investigation for future research.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Neural networks with structured layers}

In deep neural network architectures some fully-connected layers, usually responsible for final computations, are not learned (due to computational bottlenecks), but their weights are constructed randomly from the Gaussian distribution. Those layers can be then replaced by $3StructBlock$-matrices. Furthermore, fully connected random layers can be also used at the beginning of the overall pipeline and serve as a preprocessing mechanism reducing data dimensionality while preserving important signal from the data \cite{choromanska2015binary}. These can be also replaced by their structured counterparts, in particular by $3StructBlock$-matrices.

\subsection{Structured random projection trees}

Random projection trees (RPTs) are effective tools for partitioning data of low intrinsic dimensionality $d$ even if the explicit dimensionality $D$ is large. The rule of the split in each node is based on the following simple randomized procedure. A projection vectors $\textbf{g}$ are chosen uniformly at random from the unit sphere.
For each data point $\textbf{x} \in \mathbb{R}^{D}$ a projection $\textbf{g}^\top \cdot \textbf{x}$ is computed and the median $m$ of the set of projections $\mathcal{P} = \{\textbf{g}^\top \cdot \textbf{x} : \textbf{x} \in \mathcal{X}\}$ is calculated. A threshold $\theta$ is chosen as: $\theta = m + \frac{6r \Delta_{\mathcal{X}}}{\sqrt{D}}$, where $r$ is chosen uniformly at random from the interval $[-1,1]$
and $\Delta_{\mathcal{X}}$ is a diameter of the dataset $\mathcal{X}$. Note that random projections vectors can be computed in advance before data is seen. In the structured RPT setting for each level of the tree the same projection vector $\textbf{g}_{struct}$ is chosen. The set of this vectors is constructed as the set of rows of the structured matrix from the \textit{3StructBlock}-family. That significantly reduces the time for costly computations of projections. Matrix from the \textit{3StructBlock}-family is also used to replace another costly computation of $\Delta_{\mathcal{X}}$ by its approximation $\Delta^{struct}_{\mathcal{X}}$. The approximation can be obtained from structured projections in a way proposed in \cite{diff_rpt}.
\end{comment}


==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

We showed a generic computational framework relying on structured projections that can be used with a variety of machine learning algorithms to speed them up.
Some special cases of that framework (often applied as heuristics verified experimentally to work in practice) were known before, but the general picture 
and a comprehensive theoretical explanation were missing. 
Not only does the theory developed by us in this paper enable us to explain the efficiency of several special structured 
cases known so far, but it also gives efficient and compact models of computations that were not considered before for many machine learning scenarios in both random and adaptive setting.



